Fast multipole networks

Two prerequisites for robotic multiagent systems are mobility and communication. Fast multipole networks (FMNs) enable both ends within a unified framework. FMNs can be organized very efficiently in a distributed way from local information and are ideally suited for motion planning using artificial potentials. We compare FMNs to conventional communication topologies, and find that FMNs offer competitive communication performance (including higher network efficiency per edge at marginal energy cost) in addition to advantages for mobility.

==> packages.tex <==


\usepackage{arxiv}

\usepackage{booktabs} 
\usepackage{nicefrac}  
\usepackage{microtype}
\usepackage[utf8]{inputenc}

%\usepackage{enumitem}
%\usepackage{times}
%\usepackage{amsaddr}
%\usepackage[margin=1in]{geometry}

\usepackage[dvipsnames]{xcolor}
\usepackage{wrapfig}
\usepackage{multirow}

%\usepackage{url}
\usepackage{amssymb}
\usepackage{amsthm}
%\usepackage[normalem]{ulem}
%\usepackage{mathabx}
\usepackage{bbm}
\usepackage{array}
\usepackage[colorlinks=true,urlcolor=purple,
linkcolor=purple,citecolor=purple]{hyperref}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{float}


\usepackage{mathrsfs}
%\usepackage{framed}
%\usepackage{latexsym}
%\usepackage{pb-diagram}
%\usepackage[mathscr]{}
\usepackage{graphicx}
%\usepackage[all]{xy} 
\usepackage{color}

\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{thmtools,thm-restate} %%for restating results 
%\usepackage[usenames, dvipsnames]{color}

\makeatletter
\def\paragraph{\@startsection{paragraph}{4}%
  \z@\z@{-\fontdimen2\font}%
  {\normalfont\bfseries}}
\makeatother

%% TIK-Z RELATED PACKAGES
\usepackage{tikz}
\usetikzlibrary{decorations.markings, backgrounds, calc, positioning, shapes, shadows, arrows, fit, automata}
\usepackage{tikz-cd}
% Nice arrowheads
\usetikzlibrary{arrows.meta}
%\tikzset{>={Latex[length=3mm,width=2mm]}}
\tikzset{>={Latex}}


